LM-Lexicon: Improving Definition Modeling via Harmonizing Semantic Experts

We introduce LM-Lexicon, an innovative definition modeling approach that incorporates data clustering, semantic expert learning, and model merging using a sparse mixture-of-experts architecture. By decomposing the definition modeling task into specialized semantic domains, where small language models are trained as domain experts, LM-Lexicon achieves substantial improvements (+7% BLEU score compared with the prior state-of-the-art model) over existing methods on five widely used benchmarks. Empirically, we demonstrate that 1) the clustering strategy enables fine-grained expert specialization with nearly 10% improvement in definition quality; 2) the semantic-aware domain-level routing mechanism achieves higher expert efficacy (+1%) than conventional token-level routing; and 3) further performance gains can be obtained through test-time compute and semantic expert scaling. Our work advances definition modeling while providing insights into the development of efficient language models for semantic-intensive applications.

==> figure/error-cases-screenshot.tex <==
\begin{figure*}[t]
    \begin{center}{
        \subfigure[GPT-4o generation]{
            \includegraphics[width=0.46\textwidth]{figure/raw/error-cases-screenshot-gpt-4o.png}
            \label{fig:error-cases-screenshot-gpt-4o}
        }
        \subfigure[Gemini-1.5-Pro generation]{
            \includegraphics[width=0.46\textwidth]{figure/raw/error-case-screenshot-gemini.png}
            \label{fig:error-case-screenshot-gemini}
        }
    }
    \end{center}
    \vspace{-1em}
    \caption{Challenges of GPT-4o and Gemini-1.5-Pro interpreting contextual multiword expression.}
    \label{fig:error-case-screenshots}
    %\vspace{-1em}
\end{figure*}

==> figure/human_eval.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=1.02\linewidth]{figure/raw/human_eval.pdf}
  \caption{Human evaluation results.}
  \label{fig:human_eval}
  %\vspace{-1.3em}
\end{figure}

==> figure/human_eval_comparison.tex <==
\begin{figure}[t]
    \hspace{-0.3cm}
    \includegraphics[width=\linewidth]{figure/raw/human-eval-comparison.pdf}
    \caption{The upper subplot ($\uparrow$) shows our \textbf{human evaluation} results. We compare \ourmethod to 5 strong baselines across randomly selected 500 samples. The bottom subplot ($\downarrow$) presents the \textbf{GPT-4 evaluation} results, given the same 500 instances provided to humans.}
    \label{fig:human_eval_comparison_results}
  %\vspace{-1em}
\end{figure}

==> figure/llama-performance.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figure/raw/llama-performance-3d-ex.pdf}
  \caption{Test performance of \textsc{Bleu} on 3D-EX (\ourmethod versus larger dense models). We assess \textsc{Llama}-3.x models and report their 32-shot results.}
  \label{fig:llama_comparison_results}
  %\vspace{-1.25em}
\end{figure}

==> figure/overall_comparison.tex <==
\begin{figure}[t]
    \includegraphics[width=\linewidth]{figure/raw/overall-comparison.pdf}
  \caption{\textbf{Auto evaluation} results by six selected metrics. Higher is better for all metrics. Error bars show the standard deviation of the mean.}
  \label{overall_comparison_results}
  %\vspace{-1em}
\end{figure}

==> figure/scaling-semantic-expert.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\linewidth]{figure/raw/scaling-semantic-experts.pdf}
  \caption{Scaling test performance of (measuring with \textsc{Bleu}) on 3D-EX, with different number of experts.}
  \label{fig:scaling_semantic_experts}
  %\vspace{-1.3em}
\end{figure}

==> section/5_exp_results.tex <==
\section{Results and Analysis}
\label{sec:results-and-analysis}

\subsection{Main Results}
\label{subsec:major-results}
\input{table/major-exp-results}
Following the training settings in \S\ref{sec:additional-experiment-results}, our major experimental results show that \ourmethod performs well in various metrics based on golden references (Table \ref{table:main_results}). The overall results show \ourmethod outperform significantly compared with the many-shot frontier models and strong supervised methods. Our best model (\textsc{LM-Lexicon-MoE} achieves the highest performance in Wordnet, Wiki, Slang, and 3D-EX, and achives the best average performance across all five benchmarks. Moreover, to consider the compute and performance gains tradeoff, we discuss the computational cost of our methods versus compared baselines in \S\ref{sec:training-inference-cost}.

\subsection{Additional Evaluation}
\label{subsec:extended-evaluation}

%\paragraph{Memorization versus Generalization}
%To discover model capacity on generalization across different data sources (i.e., domains), we conduct extended experiments to investigate how the finetuned model trained on seen term entries can generalize to unseen entries with definition modeling. Concretely, we split the data from each domain's training set by the lexically disagreed sharding, train models separately, and test them on the test set composed of a series of unseen terms, respectively. The experimental results are shown in Figure [ref].

%\paragraph{Impact of Training Data Diversity}
%Our results show that diverse training data will help improve the modeling effect in validation loss. As shown in the Figure. The model prefers more diverse training examples, concretely, (i) the same term with multiple definitions and (ii) the same term with multiple sources. Inspired by it, we hypothesize that ``more diverse training data, modeling performance better''.

\paragraph{\ourmethod Outperforms Larger Model}
A comparison of \ourmethod to other models in Figure \ref{fig:llama_comparison_results} demonstrates that our method surpasses significantly larger dense models supervised by general instruction tuning, such as \textsc{Llama-3.3-70B-Instruct} and \textsc{Llama-3.1-405B-Instruct}, by $+30.21\%$ and $+26.13\%$ in \textsc{BLEU}, as well as $+2.1\%$ and $+1.7\%$ in \textsc{Bert Score}, respectively. In practice, we test two large dense models using the best 32-shot ICL settings. These results suggest merely scaling the model size may not enhance performance effectively in DM, and the efficacy of model specialization with our semantic-oriented sparsifying upcycling method.
\input{figure/llama-performance}

\paragraph{Impact of Test-time Compute}

In light of \citet{NEURIPS2020_1f89885d,cobbe2021training}, we are curious on how to spur \ourmethod to achieve higher performance via test-time scaling, notably ground truth-based (Oracle) and Best-of-N (BoN) sampling with a outcome verifier (ORM). For oracle verifier, it uses reference as verification to provide binary feedbacks. When the verifier operates as an ORM, it employs scalar feedback to select the optimal generation from candidates.
\input{figure/repeated-sampling-performance}
As depicted in Table \ref{table:main_results} (BoN-ORM), interestingly, it is observed that the oracle verifier is able to boost task performance (avg. $\Delta\textsc{Bleu} > 2\%$) for \textsc{LM-Lexicon-Dense}. However, it exhibits more limitations for \textsc{LM-Lexicon-MoE}; we speculate that this is because of the diversity dimishment of models, as illustrated in \cite{brown2024large}. Intuitively, optimal results are achived via oracle verifier (Fig. \ref{fig:repeated_sampling_performance}) through repeated sampling with 128 completions per test case. Collaborating with the ORM or Oracle verifiers, \ourmethod's generation quality shows consistent improvements across the five benchmarks with the increase in the number of generations. This outcome aligns with the similar findings in mathematical reasoning tasks \cite{cobbe2021training,brown2024large}.

\paragraph{Scaling In-Context Learning}
\input{figure/in-context-scaling-results}
To explore the ability and limitations of LLMs in definition modeling, we evaluated three strong models on WordNet performed across zero-, few-, and many-shot ICL.

As depicted in Figure \ref{fig:icl-scaling-results}, lexical similarities, including \textsc{Bleu} and \textsc{Rouge-L}, improve with an increasing number of shots. Moreover, the semantic similarities among  \textsc{BertScore}, \textsc{MoverScore}, and \textsc{Mauve} exhibit the same trend. However, both \textsc{GPT-4} and \textsc{Claude-3} begin to struggle with following task instructions when more $<$input, output$>$ pairs are fed. In a particular range ($k \leq 32$), task performance improves as the exemplar number increases. However, it turns to degrade when $k > 32$, which indicates \textbf{too many exemplars hurt performance, even causing model collapse owing to increasing in-context semantic contradictions.} Hence, the optimization of DM with scaled ICL is limited. This finding is contrary to recent wisdom, which claims that many-shot prompting can continuously improve the model performance on many tasks \cite{agarwal2024many,bertsch2024context,li2024long}.
%\paragraph{Impact of Fine-tuning Methods}
%\begin{gquote}
    %We investigate the factors on finetuning methods chosen to perform DM tasks. We find that the full-parameter finetuning method achieves better results than LoRA adapting and partial-parameter training. It implies that xx.
%\end{gquote}
%Different finetuning methods have different significances for DM. We conduct ad-hoc experiments for three kinds of finetuning methods: (i) full-parameters finetuning (FFT); (ii) partial-parameters finetuning (PFT); and (iii) low-rank adaptation. Through our experiments (LoRA), we find that the full parameters finetuning surpasses most of the metrics among the others.

%\input{figure/overall_comparison}
\input{figure/scaling-semantic-expert}

\subsection{Ablation Studies}
\label{subsec:ablation-study}

We conduct ablation to study the crucial factors used in \ourmethod. In particular, we controlled for three keys: 1) the data partition method, 2) the routing policy, and 3) the number of experts. % Along with the mean performance, we also provide the one-sided p-value in t-test.

%\paragraph{Prompt Choice.}\label{para:prompt-choice-ablation}
%We first ablate the factor of training on prompt $p$ used in the instruction tuning experiments. \ding{172} Alpaca-style prompt; \ding{173} longer prompt; \ding{174} prompt without task description.

% We don't need to pay attention to ablate the impact of prompt choice in the training procedure.
%\paragraph{Prompt Choice.}\label{para:prompt-choice-ablation}
%We first ablate the factor of training on prompt $p$ used in the instruction tuning experiments. \ding{172} Alpaca-style prompt; \ding{173} longer prompt; \ding{174} prompt without task description.

%\paragraph{Number of Experts $\mathcal{E}$.}\label{para:number-of-experts-ablation}
%We conduct experiments by adjusting the number of experts ($\lvert \mathcal{E} \rvert = 2, 4, 8, 16$) in \ourmethod.

\paragraph{Data Partition.}
\label{para:cluster-policy-ablation}
Since \ourmethod integrates the knowledge acquired by experts from various data partitions, our first focus is on the impact of data partition methods. To this end, we considered three settings: (i) no split, (ii) random split, and (iii) lexical split. For random split, we follow \citet{li2022branch} to slice the data into four balanced subsets and specialise an expert for each of them. For lexical split, we perform partition by TF-IDF.

As plotted in Table \ref{tab:ablation-data-partition}, we observed that the original setting with semantic embedding clustering outperforms with about $+7\%$ gains in \textsc{Bleu} and $+1\%$ gains in \textsc{Rouge} compared with lexical-based partition. The results imply that learning from semantic-targeted data clusters may help capture more precise senses and use more appropriate words to compose definitions. Lastly, it helps \ourmethod specialise robuster experts for each domain.

\input{table/ablation-data-partition}

\paragraph{Routing Policy.}
\label{para:routing-strategy-ablation}
To obtain an in-depth comprehension on the routing policies and seek more effective semantic routing mechanism. Other than top-2 token-level routing, we experiment on (i) top-1 token-level; (ii) sequence-level; and (iii) domain-level. For token-level routing, we followed the implementation of \cite{fedus2022switch} and \cite{jiang2024mixtral}. For sequence-level routing, we follow \citet{pham-etal-2023-task}. For domain-level routing, we implemented it inspired by \citet{JMLR:v22:20-1307} and \citet{gururangan-etal-2022-demix}.
\input{table/ablation-routing-policy}
Table \ref{tab:ablation-routing-policy} presents that the domain-level routing are the most effcient, even surpassing the top-2 token-level routing (\ourmethod), indicating semantic-routing by specified domain cluster may be more beneficial for semantic-intensive tasks.% As reported by \citet{shazeer2017} and \citet{zoph2022st}, with respect to the load imbalance phenomenon in \textsc{LM-Lexicon-MoE}, we leave this direction of semantic expert routing balance to future study.

\paragraph{Number of Semantic Experts.}
\label{para:expert-numbers-ablation}
Except for the aforementioned four-experts \textsc{LM-Lexicon-MoE} model, to investigate the impact of the number of semantic experts, we conduct experiments by adjusting the number of semantic experts ($N = 1, 2, 4, 8$) in \ourmethod. Notably, when $N=1$, \ourmethod collapses back to a dense model and expands to the sparse model with $N > 1$ experts.

As shown in Figure \ref{fig:scaling_semantic_experts}, we find that across all settings of $N$, our model consistently increases and outperforms the others, which are composed of fewer experts. For example, the model of $N=1$ returns $41.38\%$ while $N=8$ yields $46.86\%$ in \textsc{Bleu}. This tendency implies the effectiveness and scalability of our method utilizing more semantic experts. This increasing trend can potentially be extended by integrating more fine-grained semantic experts, as illustrated by \citet{dai-etal-2024-deepseekmoe} and \citet{he2024mixture}, but we leave this direction for future work.

%\paragraph{Mean Weights Methods}
 %In particular, we consider three popular weight-merging methods, namely LinearMerge, SLERP, and TIES, implemented by \citet{goddard2024arcee}.

%\paragraph{Trainable Modules (Optional).} We design extended experiments to ablate the factors on trainable parameters, which may affect model performance to some extent. Our analysis show that \wipinrow{}.

%\paragraph{MoE Architecture.}\label{para:system-arch-ablation}
%\ourmethod is trained with mixed MoE architecture whose MHA and MLP forward are based on 4 $\times$ branches of experts. Furthermore, we investigate the effectiveness of different MoE architectures, such as MoE with feedforward network layers parallelism (FFN MoE), MoE with attention layers parallelism (MHA MoE), and mixed layer parallelism (MHA + FFN MoE). The ablation results are shown in Table \ref{tab:ablation-moe-architecture}.

%\input{table/ablation-moe-architecture}

==> section/6_analysis.tex <==
\section{Human Evaluation}\label{sec:human_eval}
To further demonstrate the effectiveness of our method, we conduct a human evaluation and provide a qualitative analysis of a random subset of 300 samples from the 3D-EX, of which definitions are predicted by our model (\textsc{LM-Lexicon-MoE}) and the compared baselines (\textsc{LM-Lexicon-Dense} and three proprietary models). To obtain a fine-grained understanding of model-specific characteristics, we propose five criteria that are essential in the modeling and evaluation of context-sensitive lexical semantics: (i) \textit{accuracy} measures how correctly the definition captures the core semantic meaning of the word; (ii) \textit{clarity} evaluates the definition's comprehensibility and transparency in conveying meaning, focusing on how easily readers can understand the concept; (iii) \textit{conciseness} assesses whether the definition achieves optimal length without redundancy or omission; (iv) \textit{context appropriateness} measures how well the definition reflects associated contexts, situations, and pragmatic constraints of the words; (v) \textit{grammar and fluency} evaluates the grammatical correctness and naturalness of the definition. We employed three linguistic graduate students majoring in linguistics and lexicography to conduct the evaluation. The evaluators were instructed to assess each of the above criteria on a 5-point scale, where 1 indicates the poorest quality and 5 represents the highest quality.

%\input{figure/scaling-semantic-expert}
%\input{figure/human_eval}
\input{figure/semantic_scaling_and_human_eval}

Figure \ref{fig:semantic_scaling_and_human_eval} presents the human evaluation results across five criteria, showing the average scores for each model. \textsc{LM-Lexicon-MoE} consistently outperforms other models in most dimensions, with particularly strong performance of accuracy (4.6). While all models demonstrate competent performance with scores above 3.8, \textsc{LM-Lexicon-MoE} shows notable advantages in capturing contextual nuances and maintaining clarity and conciseness in definitions. The proprietary models (Claude-3-Opus, Gemini-1.5-Pro, and GPT-4-Turbo) perform similarly well but show slightly lower scores in terms of context appropriateness and conciseness than other criteria. A representative example is \textit{Word: ``coon'', Context: ``I’ll be a gone coon when the battle starts'', Reference: ``an eccentric or undignified rustic'' (from WordNet)}, in which only \textsc{LM-Lexicon-MoE} captures the correct meaning (``a person who is deemed to be despicable or contemptible''), while the other models fail to capture fundamental aspects of the reference definition.

In conclusion, while LLMs demonstrate proficiency in handling DM, they cannot fully substitute traditional dictionaries, particularly given the reliability and curation requirements in educational and professional scenarios, as well as limitations such as verbose responses and potentially toxic content from models. It is evident that LLMs have considerable potential in assisting humans in producing a sufficiently high-quality draft dictionary. This is what we advocate in this work that LLMs give rise to a new generation of tools that enhance productivity in the field of lexical semantics.

==> section/6_analysis_dep.tex <==
\section{Analysis}\label{sec:analysis}
To further demonstrate the effectiveness of our method, we conducted qualitative analysis (\S\ref{subsec:qualitative-analysis}) and human evaluation (\S\ref{subsec:human-evaluation}) on a random subset of 300 problems from the WordNet, predicted by our models, and the compared baselines.

\subsection{Qualitative Analysis}\label{subsec:qualitative-analysis}
We demonstrate the selected cases in error explanation compared to its gold standard in context and categorize them into three typical classes shown in Table \ref{tab:error_analysis_examples}.

\subsection{Human Evaluation}
\label{subsec:human-evaluation}

We employ three linguistic graduates who major in linguistics and lexicography. We query them with the training guidance and make them select the best definition from one of the options generated by several baselines. We compute the win rate and plot the confusion matrix. The Figure shows that the results of the human evaluation are $\cdots$.

The results are shown in Figure \ref{fig:human_eval_comparison_results}, it shows $\cdots$.

\iffalse
\subsection{Discussion}
\label{subsec:discussion}
In this section, we issue and dissect three research questions.

\paragraph{RQ1: Can LLMs directly answer users' lexical queries, making dictionaries useless?}
No, mainly because of reliability and curation issues for those committed users from educational and professional settings. Another limitation points to API-based proprietary models verbose answers, potentially toxic content...

\paragraph{RQ2: Can LLMs generate good dictionaries with minimal human input making lexicographers redundant?}
No. Some representative examples... 

\paragraph{RQ3: Can LLMs produce a good-enough-quality draft dictionary ready for human post-editing making the tools we use now redundant?}
Maybe yes (this is exactly what we advocate for in this work, LLMs give rise to a new generation of tools that enhance productivity.)

%\subsection{Scalability (Optional)}
%\label{subsec:scalability}
%We also promote the LLM democracy for lexical studies, to aid the development of lexicon applications such as exemplification modeling \cite{barba2021exemplification} and full-fledged dictionary writing \cite{ortega2023spanish}. \revise{More scalable aspects: \ding{172} tasks; \ding{173} data source.} Through our method, We can integrate numerous domain-specific layers into an already pre-trained transformer decoder by parallelizing it either at the MLP or MHA modules of the model. We can then freeze the parameters and learn the domain-specific components of weight. This new approach means it is straightforward to adapt pre-trained networks to a new domain by training a small number of dedicated parallel layers, and it could easily be extended to various other downstream.
\fi

==> table/ablation-moe-architecture.tex <==
\begin{table}[ht]
    \centering
    \small
    {\begin{tabular}{l|ccl}
        \multicolumn{2}{c}{} \\
        \toprule
        \textbf{Model} & \multicolumn{1}{c}{\textbf{BL}} & \multicolumn{1}{c}{\textbf{RL}} & \multicolumn{1}{c}{\textbf{BS}} \\
        \midrule
        \LogoSmall\ {\small\ourmethod} & 36.3${\scriptscriptstyle\pm}$\tiny{0.2} & 36.3${\scriptscriptstyle\pm}$\tiny{0.2} & 36.3${\scriptscriptstyle\pm}$\tiny{0.2} \\
        \midrule
        + w/ FFN MoE & 35.9${\scriptscriptstyle\pm}$\tiny{0.2} & 35.9${\scriptscriptstyle\pm}$\tiny{0.2} & 35.9${\scriptscriptstyle\pm}$\tiny{0.2} \\
        + w/ MHA MoE & 34.6${\scriptscriptstyle\pm}$\tiny{0.6} & 34.6${\scriptscriptstyle\pm}$\tiny{0.6} & 34.6${\scriptscriptstyle\pm}$\tiny{0.6} \\
        + w/ \textsc{Full} MoE & 34.0${\scriptscriptstyle\pm}$\tiny{0.2} & 34.0${\scriptscriptstyle\pm}$\tiny{0.2} & 34.0${\scriptscriptstyle\pm}$\tiny{0.2} \\
        \bottomrule
    \end{tabular}}
    \caption{Ablation results of various factors or components from four aspects defined in this paper.}
    \label{tab:ablation-moe-architecture}
\end{table}

==> table/inference-settings.tex <==
\begin{table}
 \centering
 \small
\begin{tabularx}{0.66\columnwidth}{lr}
\toprule
    \addlinespace
  \textbf{Name} & \textbf{Assignment} \\
  \addlinespace
\midrule
  \textbf{Temperature} & 0.6  \\
\addlinespace
  \textbf{Top-k} & 50  \\
\addlinespace
  \textbf{Top-p} & 0.9 \\
\addlinespace
  \textbf{typical-p} & 1.0 \\
\addlinespace
  \textbf{repetition penalty} & 1.05  \\
\addlinespace
  \textbf{max new tokens} & 64  \\
\addlinespace
  \textbf{min new tokens} & 0 \\
\bottomrule
\end{tabularx}
\caption{Decoding parameters used in the experiments.}
\label{tab:infernece-settings}
\vspace{-1em}
\end{table}

==> table/instruction-tuning-example.tex <==
\begin{table*}
    \footnotesize
    \centering
    \begin{tabular}{p{9cm}}
    \toprule
    \textbf{Word:} vibrato \\
     \textbf{Context:} He felt his teeth methodically, one after the other, with a \textcolor{purple}{vibrato} movement of finger and thumb. \\
     \textbf{Reference:} A rapid slight variation in pitch in singing or playing some musical instruments producing a stronger or richer tone. \\
     \textbf{Source:} \texttt{Wiktionary}  \\  
     \midrule
     \textbf{Instruction Tuning Example: } \\  
     \textbf{Q:} \texttt{[INST]} ``He felt his teeth methodically, one after the other, with a vibrato movement of finger and thumb'' What is the definition of ``\textcolor{purple}{vibrato}''? \texttt{[/INST]} \\
      \textbf{A:} A vibrato is a musical technique where a performer quickly and repeatedly varies the pitch of a note. \\

        \bottomrule
    \end{tabular}
    \caption{An example item of word with its exemplar context and a contextual definition. Each of data point are constructed by Q\&A format (instruction-output pair) and then feeding forward to the model in training procedure. 
    }
    \label{tab:sift-example}
\end{table*}

==> table/qualitative-analysis-details.tex <==
\begin{table*}[t]
\centering
\small
\renewcommand{\arraystretch}{1.25}
\begin{tabular}{lcp{12cm}}
\toprule
\textbf{Category} & \textbf{Model} & \textbf{Example} \\ \hline
\multirow{10}{*}{\makecell{\ding{172} Toxicity}}  
 & \multirow{2}{*}{
GPT-4} & i saw more police crime scene tape strung up by the \textbf{bunny huts}. natives must be getting restless again. $\rightarrow$ \textit{\textcolor{red}{Small, temporary shelters or huts used by people who are engaged in illicit or informal activities, such as drug dealing or other illegal activities.}} $\rightarrow$ \textcolor{OliveGreen}{housing developments, such as low-income apartment complexes, typically located in depressed urban areas.  commonly populated by black people.} \\ \cline{2-3} & \multirow{2}{*}{
Gemini-Pro} & i saw more police crime scene tape strung up by the \textbf{bunny huts}. natives must be getting restless again. $\rightarrow$ \textit{\textcolor{red}{Small dwellings or shelters used by a specific community, possibly indigenous people.}} $\rightarrow$ \textcolor{OliveGreen}{housing developments, such as low-income apartment complexes, typically located in depressed urban areas.  commonly populated by black people.} \\ \cline{2-3} & \multirow{2}{*}{
Llama-3-70b } & i saw more police crime scene tape strung up by the \textbf{bunny huts}. natives must be getting restless again. $\rightarrow$ \textit{\textcolor{red}{A housing project or residential area known for having a high concentration of Native American residents.}} $\rightarrow$ \textcolor{OliveGreen}{housing developments, such as low-income apartment complexes, typically located in depressed urban areas.  commonly populated by black people.}
   \\ \bottomrule
\end{tabular}
\caption{An example for each error category.}
\label{tab:error_analysis_examples}
\end{table*}
